Molecule survival in magnetized protostellar disk winds. II. Predicted H2O line profiles versus Herschel/HIFI observations

We investigate whether the broad wings of H2O emission identified with Herschel towards low-mass Class 0 and Class 1 protostars may be consistent with an origin in a dusty MHD disk wind, and the constraints it would set on the underlying disk properties. We present synthetic H2O line profiles predictions for a typical MHD disk wind solution with various values of disk accretion rate, stellar mass, extension of the launching area, and view angle. We compare them in terms of line shapes and intensities with the HIFI profiles observed by the WISH Key Program. We find that a dusty MHD disk wind launched from 0.2--0.6 AU AU to 3--25 AU can reproduce to a remarkable degree the observed shapes and intensities of the broad H2O component, both in the fundamental 557 GHz line and in more excited lines. Such a model also readily reproduces the observed correlation of 557 GHz line luminosity with envelope density, if the infall rate at 1000 AU is 1--3 times the disk accretion rate in the wind ejection region. It is also compatible with the typical disk size and bolometric luminosity in the observed targets. However, the narrower line profiles in Class 1 sources suggest that MHD disk winds in these sources, if present, would have to be slower and/or less water rich than in Class 0 sources. In conclusion, MHD disk winds appear as a valid (though not unique) option to consider for the origin of the broad H2O component in low-mass protostars. ALMA appears ideally suited to further test this model by searching for resolved signatures of the warm and slow wide-angle molecular wind that would be predicted.

==> aliases.tex <==
% \newcommand{\apj}{ApJ}
% \newcommand{\aap}{A\&A}
% \newcommand{\apjl}{ApJL}
% \newcommand{\mnras}{MNRAS}

\newcommand{\eab}{\begin{array}} \newcommand{\eae}{\end{array}}
\newcommand{\eqab}{\begin{eqnarray}} \newcommand{\eqae}{\end{eqnarray}}
\newcommand{\eqb}{\begin{equation}} \newcommand{\eqe}{\end{equation}}

\newcommand{\sub}{\mathrm{sub}}

\newcommand{\water}{\mathrm{H}_\mathrm{2}\mathrm{O}}
\newcommand{\CO}{\mathrm{C}\mathrm{O}}
\newcommand{\HH}{\mathrm{H}_\mathrm{2}}
\newcommand{\OH}{\mathrm{OH}}

\newcommand{\Macc}{$\dot M_{\rm acc}$}
\newcommand{\Msun}{$M_\odot$}
\newcommand{\Mstar}{$M_\star$}
\newcommand{\romax}{$r_{0}^\mathrm{max}$}
\newcommand{\romin}{$r_{0}^\mathrm{min}$}
\newcommand{\Lbol}{$L_{\rm bol}$}
\newcommand{\Lacc}{$L_{\rm acc}$}
\newcommand{\Lstar}{$L_\star$}
\newcommand{\Tkin}{$T_\mathrm{kin}$}
\newcommand{\Tdust}{$T_\mathrm{d}$}
\newcommand{\Tbol}{$T_\mathrm{bol}$}
\newcommand{\Rsub}{$R_\sub$}


\newcommand{\TdV}{$\int TdV$\,}

\newcommand{\mMstar}{M_\star}
\newcommand{\mMacc}{\dot M_{\rm acc}}
\newcommand{\mMsun}{M_\odot}
\newcommand{\Rsun}{R_\odot}
\newcommand{\Lsun}{L_\odot}
\newcommand{\Lhs}{L_{\mathrm{hs}}}
\newcommand{\Rstar}{R_\star}
\newcommand{\Tstar}{T_\star}
\newcommand{\Tex}{T_\mathrm{ex}}
\newcommand{\Ltot}{L_{\rm tot}}

\newcommand{\UMacc}{\mathrm{M_\odot}~\mathrm{yr}^{-1}}

\newcommand{\vgrad}{\frac{\partial V}{\partial s}}
\newcommand{\nH}{$n_\mathrm{H}$}
\newcommand{\nHH}{$n_{\mathrm{H}_2}$}
\newcommand{\nff}{$n^\mathrm{ff}_{\mathrm H_2}$}
\newcommand{\nenv}{$n^\mathrm{env}_{\mathrm H_2}$}

\newcommand{\AAr}{\mathrm{\AA}}
\newcommand{\abs}{\mathrm{abs}}
\newcommand{\acc}{\mathrm{acc}}
\newcommand{\ad}{\mathrm{ad}}
\newcommand{\adia}{\mathrm{adia}}
\newcommand{\AU}{\mathrm{AU}}
\newcommand{\bl}{\mathrm{bl}}
\newcommand{\gra}{\mathrm{gra}}
\newcommand{\Cr}{\mathrm{C}}
\newcommand{\cm}{$\mathrm{cm}^{-3}$}
\newcommand{\dr}{\mathrm{d}}
\newcommand{\D}{\mathrm{D}}
\newcommand{\er}{\mathrm{e}}
\newcommand{\eff}{\mathrm{eff}}
\newcommand{\emr}{\mathrm{em}}
\newcommand{\erg}{\mathrm{erg}}
\newcommand{\eV}{\mathrm{eV}}
\newcommand{\ext}{\mathrm{ext}}
\newcommand{\Hr}{\mathrm{H}}
\newcommand{\He}{\mathrm{He}}
\newcommand{\Hz}{\mathrm{Hz}}
\newcommand{\GHz}{\mathrm{GHz}}
\newcommand{\ir}{\mathrm{i}}
\newcommand{\inr}{\mathrm{in}}
\newcommand{\K}{\mathrm{K}}
\newcommand{\keV}{\mathrm{KeV}}
\newcommand{\km}{\mathrm{km}}
\newcommand{\m}{\mathrm{m}}
\newcommand{\minr}{\mathrm{min}}
\newcommand{\maxr}{\mathrm{max}}
\newcommand{\n}{\mathrm{n}}
\newcommand{\N}{\mathrm{N}}
\newcommand{\Or}{\mathrm{O}}
\newcommand{\p}{\mathrm{p}}
\newcommand{\pe}{\mathrm{pe}}
\newcommand{\pc}{\mathrm{pc}}
\newcommand{\rr}{\mathrm{r}}
\newcommand{\s}{\mathrm{s}}
\newcommand{\sh}{\mathrm{sh}}
\newcommand{\sr}{\mathrm{sr}}
\newcommand{\sca}{\mathrm{sca}}
\newcommand{\sil}{\mathrm{sil}}
\newcommand{\UV}{\mathrm{uv}}
\newcommand{\IR}{\mathrm{ir}}
\newcommand{\yr}{\mathrm{yr}}
%
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\vb}{\mathbf{v}}
%
\newcommand{\Bv}{\vec{B}}
\newcommand{\Jv}{\vec{J}}
\newcommand{\rv}{\vec{r}}
\newcommand{\vv}{\vec{v}}
\newcommand{\uu}{\vec{u}}
\newcommand{\kms}{\rm{km~s}$^{-1}$}

